Leveraging Logical Rules in Knowledge Editing: A Cherry on the Top

Multi-hop Question Answering (MQA) under knowledge editing (KE) is a key challenge in Large Language Models (LLMs). While best-performing solutions in this domain use a plan and solve paradigm to split a question into sub-questions followed by response generation, we claim that this approach is sub-optimal as it fails for hard to decompose questions, and it does not explicitly cater to correlated knowledge updates resulting as a consequence of knowledge edits. This has a detrimental impact on the overall consistency of the updated knowledge. To address these issues, in this paper, we propose a novel framework named RULE-KE, i.e., RULE based Knowledge Editing, which is a cherry on the top for augmenting the performance of all existing MQA methods under KE. Specifically, RULE-KE leverages rule discovery to discover a set of logical rules. Then, it uses these discovered rules to update knowledge about facts highly correlated with the edit. Experimental evaluation using existing and newly curated datasets (i.e., RKE-EVAL) shows that RULE-KE helps augment both performances of parameter-based and memory-based solutions up to 92% and 112.9%, respectively.

==> section/1a_introduction.tex <==
\section{Introduction}
\asif{Large Language Models (LLMs) have powerful reasoning and comprehension 
capabilities for worldly knowledge~\cite{Wei2022ChainOT,Huang2022TowardsRI}. 
This capability enable LLMs to easily answer multi-hop questions (MQA), which require multiple reasoning steps \cite{Lan2021ASO,Mavi2022ASO} and extensive 
open-domain knowledge. 
However, the end-performance of LLMs is still limited by incorrect and/or 
outdated knowledge, due to which they tend to generate plausible yet 
incorrect answers for unknown facts, a phenomenon known 
as hallucinations~\cite{Hong2023FaithfulQA}.
The LLMs show very limited adaptability to newly emerging information and 
knowledge, which greatly undermines the reliability of LLMs for MQA.
Updating the LLMs information/knowledge through retraining is 
computationally demanding making timely edits impossible. 
MQA under knowledge editing (KE), which aims to provide answer to the multi-hop question based on given fact edits, has thus become a popular research area in artificial intelligence \cite{zhong2023mquake,gu2023pokemqa}.}


\asif{There are two dominant research directions for this area, i.e., parameter-based editing and memory-based editing. The parameter-based editing methods update the knowledge in LLMs by modifying parameters of model. 
Some examples in this regard include ROME~\cite{meng2022locating} and its improved variant MEMIT by Meng et al.,~\cite{meng2022mass}.
On the contrary, the memory-based editing methods explicitly maintain a 
memory to store the information about the knowledge and facts to be modified. Examples include MeLLo by Zhong et al.,~\cite{zhong2023mquake}, and PokeMQA by Gu et al.,~\cite{gu2023pokemqa}.
These methods primarily adopt the plan-and-solve 
paradigm~\cite{Khot2022DecomposedPA, Wang2023PlanandSolvePI}, where 
LLMs are prompted to decompose multi-hop question into sub-questions, 
then iteratively interact with edit memory to solve each sub-question.
Generally, the memory-based approaches perform better than the 
parameter-based approaches, because the former approach is not flexible 
to incorporate the reasoning required to solve complex questions \cite{zhong2023mquake}.}


\asif{
We observe that the existing memory-based methods 
rely on LLMs for their planing stage. 
\eat{face a key challenge explained as follows. 
These approaches rely on LLMs for the planning stage,}
And, in most of the cases LLMs tend to generate an 
overly-concise/coarse-grained \eat{and concise }plan. 
These coarse-grained plans are not only hard to follow but 
may eventually lead to false response for multi-hop 
questions thus limiting the end-performance of the model.}


\warn{This is also illustrated in Figure \ref{fig:challenge}, 
which shows``Who is the boss of Tom?'' is a coarse-grained sub-question. This sub-question relies on multiple fine-grained 
knowledge about Tom's company and company's owner. 
If edits occurs in this knowledge, it will cause 
\textit{ripple effects}, and the direct knowledge of \warn{the coarse-grained sub-question} will be affected accordingly. Existing memory-based method use the dense retrieval to get the semantic relevance of the sub-question and edit. However, the relevance score between coarse-grained question and the two edit are low because the edit is not directly related to the sub-question. This issue results in fail to find the edit. Moreover, a problem related to multiple edits also cause trouble, and all the edit needs to be given to LLM for reasoning. Existing memory-based method lacks direct coarse-grained edit to this coarse-grained sub-question thus resulting in easy answer failure.}


\eat{The rule has been widely studied in the knowledge graph reasoning (KGR) task and is used to complete the knowledge graph by combining existing knowledge \cite{Tang2022RulENK}.
\textbf{Black-box LLMs inevitably generate shortcuts plan, so we can imitate KGR and use rule to generate coarse-grained edits to improve accuracy in solving coarse-grained sub-question.}}



To address the aforementioned challenges, we propose a novel method~\OurMODEL{}: \underline{\textbf{K}}nowledge \underline{\textbf{E}}diting based on \underline{\textbf{\textsc{Rule}}}. 
~\OurMODEL{}\eat{analyzes and solves the key challenges from the 
perspective of logic rules. Specifically, it} uses 
\textit{First-order Logic} (FOL) rules to generate coarse-grained 
edits to improve accuracy in solving coarse-grained 
sub-questions.\fixme{Mention Horn Rule here..!}

\warn{FOL uses the universal quantifier to represent generally applicable logical rules, e.g., "$\forall x,y,z:$ $x$'s company is $y$ $\land$ $y$’s owner is $z$ $\rightarrow$ $x$'s boss is $z$". When the rules are given explicitly,~\OurMODEL{} traverses the rules for the newly added edits, and then generates new coarse-grained edits based on the matching rules. For example, we can generate a coarse-grained edit "The boss of Tom is Elon Musk" for the two edit about company and owner in figure 1. Then this new generated edit can directly edit the coarse-grained question, result in high semantic relevance and no need to worry one sub-question may related to two edit.}
When the rules are not given explicitly,~\OurMODEL{} adopt a  rule-free technique to semantically merge two \warn{consecutive edits.}
~\OurMODEL{} is a plug-and-play model that can be easily/flexibly integrated with any memory-based methods.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Figure/Challengeplan.pdf}
    \vspace{-1.7ex}
    \caption{\warn{\textbf{The example of coarse-grained plan.} We observe that LLMs tend to generate a coarse-grained plan (the left side). The left side is better than the right side, because the edit directly modify the knowledge of the sub-question, therefore the semantic relevance score is high between them, and one sub-question is only realted to one edit.}}
    \label{fig:challenge}
    \vspace{-3.7ex}
\end{figure}
Experimental evaluation using the benchmark data sets shows that~\OurMODEL{} surpasses the existing methods by a significant 
margin. \eat{achieving state-of-the-art performance.}
Given that, existing datasets do not explicitly provide 
set of rules, we also introduce a new evaluation benchmark, 
namely: \underline{\textbf{R}}ule-aware MQA \underline{\textbf{u}}nder \underline{\textbf{K}}nowledge \underline{\textbf{E}}diting (\textsc{RuKE}) that
encompasses a set of rules along with multi-hop questions.

\warn{The two settings provide a comprehensive evaluation of the knowledge editing method to solve ripple effects.}
We summarize the key contributions of our work as follows:

\begin{itemize}
    \item We propose~\OurMODEL{} that uses logic rules to overcome 
    the limitations of the \eat{systematically analyze the hazards of} coarse-grained knowledge editing plans generated by LLMs.
    \item \warn{We propose a new multi-hop question based on the knowledge editing benchmark, explicitly giving the rules.}
    \item \warn{We propose~\OurMODEL{} and a rule-free technique,
    ~\OurMODEL{} greatly surpasses previous methods.}
\end{itemize}






\eat{
For planing stages these approaches rely on 
They rely on the in planning stage: 
LLMs tend to generate \textit{plan shortcut} which include coarse-grained 
sub-question that easily fails to answer.}


\eat{Thus, we launch a new benchmark and set whether to provide rules.} 





\eat{We observe that existing memory-based methods face a key challenge in planning stage: 
LLMs tend to generate \textit{plan shortcut} which include coarse-grained 
sub-question that easily fails to answer. 
As Figure \ref{fig:challenge} 
shows, ``Who is the boss of Tom?'' is a coarse-grained sub-question. 
This sub-question relies on multiple fine-grained knowledge about Tom's 
company and its owner. 
If edits occurs in this knowledge, it will cause 
\textit{ripple effects}, and the direct knowledge of the sub-question will 
be affected accordingly. 
Existing memory-based method lacks direct edit 
to this sub-question thus resulting in easy answer failure. 
We analyze 
and solve this challenge from the perspective of logic rule:
\textit{First-order Logic} uses the universal quantifier to represent generally applicable logical rules, e.g., "$\forall x,y,z: y$ is $x$'s company, $z$ is $y$’s owner $\rightarrow z$ is $x$'s boss" \fixchen{citation need}. We refer to First-order Logic as \textit{rule} for simplicity. The rule has been widely studied in the knowledge graph reasoning (KGR) task and is used to complete the knowledge graph by combining existing knowledge \cite{Tang2022RulENK}. \textbf{Black-box LLMs inevitably generate plan shortcuts, so we can imitate KGR and use rule to generate coarse-grained edits to improve accuracy in solving coarse-grained sub-question.} 
To address the aforementioned challenge, we propose a novel method \textsc{KeRule}: \underline{\textbf{K}}nowledge \underline{\textbf{E}}diting based on \underline{\textbf{Rule}}. When the rule is given explicitly, \textsc{KeRule} traverses all matching rules for the newly added edits and obtains coarse-grained edits. When the rule is not given explicitly, \textsc{KeRule} adopt a  rule-free technique to semantically merge two consecutive edits. \textsc{KeRule} is plug-and-play and can be simply used for any memory-based method.
We evaluate \textsc{KeRule} on existing datasets. Experimental results show that \textsc{KeRule} greatly surpasses existing methods and achieves state-of-the-art performance. Existing datasets do not explicitly provide rules. Thus, we launch a new benchmark and set whether to provide rules. The two settings provide a comprehensive evaluation of the knowledge editing method to solve ripple effects. Our contributions are summarized as follows:
\begin{itemize}
    \item We introduced logic rules to systematically analyze the hazards of coarse-grained plans that large models tend to generate. 
    \item We propose \textsc{KeRule} and a rule-free technique, \textsc{KeRule} greatly surpasses previous methods.
    \item We propose a new multi-hop question based on the knowledge editing benchmark, explicitly giving the rules.
\end{itemize}
}

==> section/3_Task.tex <==



==> section/4a_Approach2.tex <==
\section{\textbf{R}easoning on Inference Path \textbf{w}ith \textbf{E}diting \textbf{F}using}
\subsection{Question decomposition and Inference Path}
As the figure 2 show, previous work adopt Step-by-step strategy, \textsc{RwEF} adopt All-at-once strategy.\\
\textbf{Step-by-step.}\cite{Aoki2023EmpiricalIO} Previous work \cite{zhong2023mquake,gu2023pokemqa} use LLMs to decompose multi-hop questions $Q$ into sub-questions $q_i$, where each $q_i$ takes the form like "What is the $r_i$ of the $s_i$?", they adopt Step-by-step strategy to generate the $q_i$, because $q_i$ can only be generated when $s_i$ is determined. \\
%\textbf{All-at-once.} The plan of \textsc{RwEF} is a  \textit{inference path} $P_{infer}$, which have the form as $\langle(s_1,r_1,o_1^\prime),\cdots,(s_n^\prime,r_n,o_n^\prime)\rangle$, where $s_i^\prime$ and $o_i^\prime$ represented their type. For instance, the type for the U.S. is country. \textsc{RwEF} can directly generate complete plans in All-at-once style, which helps distill planning capabilities into small models. One example of the inference path for the question "Who is the owner of the company of Tom?" is: 
\textbf{All-at-once.} The plan of \textsc{RwEF} adopt \textit{inference path}: $P_{Q} = s_1 \xrightarrow{r_1} o_1^\prime \xrightarrow{r_2} \cdots \xrightarrow{r_n} o_n^\prime$, where $o_i^\prime$ denote category for $o_i$. For example, the inference path for the question "Who is the owner of the company of Tom?" is: $\text{Tom}\xrightarrow{\text{company\_is}}\text{compnay}\xrightarrow{\text{owner\_is}} \text{people}$. \textsc{RwEF} can directly generate complete plans in All-at-once style.

\subsection{Planning and Reasoning on Inference path}
%我们使用ICL通过LLMs将问题转换为推理路径。首先写几个高质量的转换成路径的demonstration, 然后加上具体的instruction, 具体可以在附录中查看.
In this section, we introduce the two stages of \textsc{RwEF}: 1) Planning. This stage \textsc{RwEF} use a language model as planner $\mathbf{M_{planner}}$ to generate a complete plan for multi-hop question $q$. 2) Reasoning. This stage \textsc{RwEF} employ a language model $\mathbf{M_{query}}$ to answer question without edit and a retrieval $\mathbf{R_{edit}}$ to find relevant edit, step-by-step solve the plan. \\
\\
\textbf{Stage1 Planning Inference Path.} \textsc{RwEF} use the $\mathbf{M_{planner}}$ module to generate inference path $P_{infer}$ and extract the time $t$ of the $q$. 
\begin{equation}
   t, P_{infer} = \mathbf{M_{planner}}(prompt\oplus q)
    \label{eq:planner}
\end{equation}
where $\oplus$ denotes the concatenation, and the $prompt$ includes five high-quality demonstrations handwritten by humans, which can be found in the appendix. We use \textit{gpt-turbo-3.5-instruct} as \textit{planner} $\mathbf{M_{planner}}$.\\
\\
%The reasoning ability of the small language model is weak. Therefore, we attempt to distill the planning capabilities of gpt into the smaller model.\\
%每一个inference path会有一个已知的起点, 然后我们会在这个路径上不断迭代式的推理。每一步推理首先检索是否有相关的editing, 如果没有找到就使用大模型进行回答。
\textbf{Stage2 Reasoning on Inference Path.} Reasoning is to derive the answer for one step of $P_{infer}$. Specifically, at the $i$-th step $(s_i^\prime,r_i,o_i^\prime)$ of the $P_{infer}$, Reasoning is to derive the specific value of $o_i$ base on the answer $s_i$ of previous step.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figure/framework4.pdf}
    \caption{\textbf{Reasoning on Relation Path with Edit Fusion}.}
    \label{fig:enter-label}
\end{figure}



Suppose we are currently at step i of reasoning. As the algorithm 1 show, we first need to determine whether this step has been edited. Thus, \textsc{RwEF} use the $\mathbf{R_{edit}}$ module retrieve the relevant edit: 
\begin{equation}
   edit, sim = \mathbf{R_{edit}}(s_i,r_i,o_i^\prime,t)
    \label{eq:retrieve}
\end{equation}
where $edit$ is the edit that most associated to this step, and $sim$ is denote the similarity. If there is no corresponding edit, we use $\mathbf{M_{query}}$ to find the answer. 
\begin{equation}
   o_i=
\begin{cases}
edit[o] & edit !=None \And sim>0.5\\
\mathbf{M_{query}}(s_i,r_i,o_i^\prime,t)& edit==None\ \| \ sim<=0.5
\end{cases}
    \label{eq:retrieveanswer}
\end{equation}
where $None$ denote that relevant edit is not found. Then we iterate the above process, $o_l$ is the final answer.


%where $\mathbf{R_{edit}}$ is the retrieval used to find the relevant editing $e$ and return the $similarity$. If editing $e$ is not found or the similarity is low, we can consider that there is no editing related to this inference step. 

%where $\mathbf{M_{query}}$ is the language model storing the knowledge before the editing. And iterative the above reasoning step along the inference path, we can get the final answer $f(o_l)$ for the multi-hop question $q$.  


\definecolor{mygreen}{RGB}{70,130,180}

\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H] 
    \caption{\scshape Reasoning on Path }
    \label{algorithm1}
    \begin{algorithmic}[1]
    \Require
        \item[] {\color{mygreen} \#$P_{inference}:$ The inference path used for reasoning}
        \item[] {\color{mygreen} \#$\mathbf{M_{query}}:$ Language models which storing knowledge before editing}
        \item[] {\color{mygreen} \#$\mathbf{R_{edit}}:$ Retrieval used to find editing}
    \Ensure answer for the question
        \State $l= Length(P_{inference})$
        \State {\color{mygreen}\# Iteratively reasoning on inference path}
        \For{$s_i, r_i, o_i$ in $P_{inference}$}
            \State {\color{mygreen}\# Retrieve the relevant editing}
            \State e, similarity = $\mathbf{R_{edit}}(f(s_i), r_i, o_i)$
            \State $\mathbf{If}$ $e = None$ or similarity<0.5:
            \State \qquad $f(o_i)$ = $\mathbf{M_{query}}(f(s_i), r_i, o_i)$
            \State $\mathbf{Else}$:
            \State \qquad $f(o_i)$ = edit.o
            \State  $f(s_{i+1}) = f(o_i)$ 
        \EndFor
        \State \Return $f(o_{l})$
    \end{algorithmic}
\end{algorithm}
\end{minipage}
   \hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \caption{\scshape Editing Fusion}
    \label{algorithm2}
    \begin{algorithmic}[1]
    \Require
        \item[] {\color{mygreen} \#$E:$ A list of requested editing}
        \item[] {\color{mygreen} \#$G_{editing}:$ The knowledge editing graph}
    \Ensure $G_{editing}$
    \State {\color{mygreen}\# fusion the 2-hop edit}
        \For{$e_i$ in $E$}
        \State $G_{editing}$.insert($e_i$)
        \For{$e_j$ in $range(E)$}
            \State $\mathbf{If}$ $e_i = e_j\ or \ e_i.o != e_j.s$:
            \State \qquad continue
            \State {\color{mygreen}\# Combien the two editing}
            \State $e_{fusion}.s=e_i.s$
            \State $e_{fusion}.o=e_j.o$
            \State $e_{fusion}.r=e_i.r + e_j.r$
            \State $G_{editing}$.insert($e_{fusion}$) 
        \EndFor
        \EndFor
        \State \Return $G_{editing}$
    \end{algorithmic}
\end{algorithm}
\end{minipage}



\section{Edit Database and Editing Fusion}
In this section, we introduce the edit database $\mathcal{D}$ used by \textsc{RwEF}. This database $\mathcal{D}$ is divided into four dimensions to store fact edits $\mathcal{E}$ , and employ a retrieval $\mathbf{R_{edit}}$ to use different retrieve rule in each dimension. Specifically, the retrieval $\mathbf{R_{edit}}$ can be divided into two steps: 1) Filter: Filter out the edits that do not meet the required subject and time limit. 2) Rerank: Rerank remaining edits based on semantic similarity.
%Due to the non-uniqueness of reasoning paths and the existence of skipping phenomena, we need a broader span of editing, where the span refers to the combination of multiple relations. We maintain a knowledge editing graph $G_{editing}$, where each node can serve as a subject or object, and each edge is a directed edge with a specific relation. If some datasets represent editing in the form of natural language sequence. We need to convert the editing $e_i$ into a triplet form $(s_i, r_i,o_i)$. For two connected editings in the graph, we can obtain a combined editing between them based on transitivity. In the ideal scenario, we could compute the transitive closure of $G_{editing}$, but this would introduce significant retrieval overhead.

%With the increasing number of edits, accurately identifying the corresponding editing poses a challenge. The previous sub-question decomposition method retrieves the editing directly from the sub-question, in which performance is not optimal. One reason is that the sub-problem has a different form from editing, while we standardize the sub-problem and editing into the same $(s,r,o)$ format. Another reason is that they encode editing in the form of complete natural language sequences, whereas we design rules based on three different dimensions $s,r,o$ for retrieval.

\subsection{Edit Database}
Previous work ignore the structure of edit, resulting in low retrieval performance. The retrieval $\mathbf{R_{edit}}:(s_i,r_i,o_i^\prime,t) \rightarrow edit,sim$ aims to find the most relevant edit in $\mathcal{D}$. That is to say, we need to find the edit where corresponding to subject entity $s_i$, the relation is $r_i$, the modification time is less than $t$, and the object type is $o$. Specifically, $\mathbf{R_{edit}}$ retrieve according to the following two steps: 

\textbf{Step1 Filter based on subject and time.} $\mathbf{R_{edit}}$ initially employed the subject $s$ and time $t$ dimension for filtering, identifying edits $e$, in which $e[s]$ is identical to the subject $s_i$ of the key and $e[t]$ is less than the time $t$. 
\begin{equation}
   \mathcal{D}_{sub} = \{e\mid e \in \mathcal{D} \ \& \ e[s] = s_i \ \& \ e[t]<t\}
    \label{eq:Re1}
\end{equation}
where $\mathcal{D}_{sub}$ is the remaining edits.\\
\\
\textbf{Step2 Rerank based on relation and object.} Then, $\mathbf{R_{edit}}$ retrieve based the relation $r$ and object $o$ dimensions. $\mathbf{R_{edit}}$ employ an encoder to get the vector embedding $v_{q}$ and $V_{editing}$ of the key and remaining edits $\mathcal{D}_{sub}$:
\begin{equation}
   v_{q}=Encoder(s_i\oplus r_i \oplus o_i^\prime)
    \label{eq:Ret1}
\end{equation}
\begin{equation}
   V_{edits}=\{Encoder(e[s]\oplus e[r] \oplus Type(e[o]))\mid e \in \mathcal{D}_{sub}\}
    \label{eq:Ret2}
\end{equation}
Where $Type(e.o)$ denotes the type of editing object $e.o$. We use cosine similarity to measure the similarity between vectors, selecting the highest similarity as the retrieval result.
\begin{equation}
    e_{result},cosine(v_{result},v_q) = \argmax_{e_i,v_i \in \mathcal{D}_{sub},V_{edits}} {\frac{v_q \cdot v_i}{\lVert v_q \rVert \lVert v_i \rVert}}
    \label{eq:Ret3}
\end{equation} 
where $e_{result}$ is the most relevant edit, and $cosine(v_{result},v_q)$ is the similarity between the key and this edit $e_{result}$.

\subsection{Editing Fusion}
Editing Fusion aims to address the challenge of plan skipping.

==> section/Cache3Approach.tex <==
\section{\OurMODEL{} \eat{Knowledge Editing based on Rule}}


In this section, we introduce the workflow of \textsc{KeRule}. \textsc{KeRule} is focus on editing processing, and can be seamlessly integrated into any backbone knowledge editing method. 

There are two ways to use \textsc{KeRule}, depending on whether to explicitly give the rule. If the rule is given explicitly, new edits are added continuously and the rule memory will be traversed to find activated rules to infer derived knowledge. If no rule is given, the two consecutive edits are semantically merged in all-edited scenario.



\subsection{\warn{Knowledge Discovery via Horn Rules}}
We leverage the horn rules to help discover novel facts/relational
instances by considering the updates originating from knowledge editing and associated ripple effects.
We refer to the newly discovered facts as the \textbf{derived knowledge}.
\fixchen{Here Write details about chase, i.e., how you use the horn rules iteratively to help discover new knowledge after KE + ripple effects...!}

\textbf{Discover Activating Horn Rule Sets.} We first



\subsection{Rule-based \textsc{KeRule}}
As illustrated in Figure \ref{fig:framework}, this section introduce how to obtain the derived knowledge in rule-based scenario.

Given a collection of fact edits $\mathcal{E}=\{e_1,e_2,\cdots\}$ and a collection of rule $\mathcal{R}=\{\varphi_1,\varphi_2, \cdots\}$, We need to obtain all the derived knowledge $\mathcal{K}_{derived}$. Taking into account real-life application scenarios, edits are added gradually. Therefore, we iteratively traverse $\mathcal{E}$ to continuously add edit $e_i$. 

For newly added edits $e=(s,r,o\rightarrow o^*)$, we obtain new knowledge $r(s,o^*)$. We first traverse $\mathcal{R}$ to find the \textbf{left-activating rule set} $\mathcal{R}_L$ and the \textbf{right-activating rule set} $\mathcal{R}_R$ for $r(s,o^*)$:
\begin{equation}
   \mathcal{R}_L = \{\textsc{r}|\textsc{r}[r_1]=r \wedge\textsc{r}\in \mathcal{R} \}
    \label{eq:lp}
\end{equation}
\begin{equation}
   \mathcal{R}_R = \{\textsc{r}|\textsc{r}[r_2]=r\wedge\textsc{r}\in \mathcal{R} \}
    \label{eq:rp}
\end{equation}
where r is the relation of the edit $e$. We generate derived knowledge for these two activated rule sets respectively.

\paragraph{Left-activating rule set.} To aid understanding, we denote edited knowledge $r(s,o^*)$ as $r_1(\alpha,\beta^*)$. We traverse rule $\textsc{r}$ on $\mathcal{R}_L$ to get derived knowledge for each rule $\textsc{r}$. We first need to determine whether there is edited knowledge $r_2(\beta^*,\gamma^*)$ right to activate $\textsc{r}$. If $r_2(\beta^*,\gamma^*)$ is existing, we obtain the derived knowledge $k_{derived}=\textsc{r}[r_3](\alpha,\gamma^*)$ in both-edited situation. If $r_2(\beta^*,\gamma^*)$ is not exist, we need to find the obejct $\underline{\gamma^*}$ by LLMs:

\begin{figure}
    \centering   
    \includegraphics[width=1\linewidth]{Figure/Ruleframework3.pdf}
    \vspace{-2.7ex}
    \caption{The framework of~\OurMODEL{}.}
    \vspace{-2.7ex}
    \label{fig:framework}
\end{figure}

\begin{equation}
   \underline{\gamma^*} = LLMs(Prompt_R(\textsc{r}[r_2],\beta^*))
    \label{eq:ql}
\end{equation}

Where $Prompt_R$ converts it into a natural language form to query the object $\underline{\gamma^*}$, which can be found in the appendix \ref{}. Then, the derived knowledge is $k_{derived}=\textsc{r}[r_3](\alpha,\underline{\gamma^*})$.

\paragraph{Right-activating rule set} To aid understanding, we denote edited knowledge $r(s,o^*)$ as $r_1(\beta,\gamma^*)$. we traverse rule $\textsc{r}$ on $\mathcal{R}_R$  to get derived knowledge for each rule $\textsc{r}$. We first need to determine whether there is edited knowledge $r_1(\alpha^*,\beta)$ left to activate $\textsc{r}$. If $r_1(\alpha^*,\gamma)$ is existing, we obtain the derived knowledge $k_{derived}=\textsc{r}[r_3](\alpha^*,\gamma^*)$ in both-edited situation. If $r_1(\alpha^*,\beta)$ is not exist, we need to find the whether subject $\underline{\alpha^*}$ by LLMs:

\begin{equation}
   \underline{\alpha^*} = LLMs(Prompt_L(\textsc{r}[r_1],\beta))
    \label{eq:qr}
\end{equation}

Where $Prompt_L$ converts it into a natural language form to query the subject $\underline{\alpha^*}$, which can be found in the appendix \ref{}. Then, the derived knowledge is $k_{derived}=\textsc{r}[r_3](\underline{\alpha^*},\gamma^*)$.

If the answer cannot be found using LLMs in the above two situations, it will be deemed. We finally construct the $\mathcal{K}_{derived}$ for all the derived knowledge $k_{derived}$. 

\subsection{Rule-free \textsc{KeRule}}
For situations where the dataset is not explicitly given a rule, we propose a simple and effective method to solve the both-edited situation. One simple implementation is to use a double loop to enumerate $\mathcal{E}=\{e_1,e_2,\cdots\}$:

\begin{equation}
   \mathcal{K}_{derived} = \{k_{derived}=(e_l[s],r_{derived},e_r[o])|e_l\in \mathcal{E} \wedge e_r\in \mathcal{E}\wedge e_l[o]=e_r[s]  \}
   \label{eq:ql}
\end{equation}

where $r_{derived}$ is concatenating by the relation of $e_l[r]$ and $e_l[r]$. We find that by simply concatenating them and then using semantic-based retrieval.

\subsection{Plan-and-solve}
~\OurMODEL{} is plug-and-play and can be applied for any plan-and-solve based method in 
MQAuKE tasks. However, ~\OurMODEL{} generates more edits, which increases the burden on 
the retrieval. Therefore, an efficient retriever is more suitable to be combined with~\OurMODEL{}.



==> section/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clearly introduce the contribution of our paper is using rules to augment existing knowledge editing methods.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitation is discussed in the final section of appendix \ref{limit}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper is not for the theoretical research but focus more on application on larger language models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the details about how to reproduce the experiment is shown in experiment setting \ref{EXP:Seting}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We plan to open access to the data and code after we sort out all the data, and will update to Github repository.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have specify all the training and test details in experiment setting \ref{EXP:Seting}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have conducted experiment multiple times to alleviate the error generated from calling API, hardware, and so on.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please see the computer resources setting on experiment setting \ref{EXP:Seting}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have discuss the potential societal negative impact due the outdated knowledge of model, and propose method to solve it.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not propose such risk data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the data we use is public-resource in Internet.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide a new datasets and they are well documented.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

